Do Audio-Language Models Understand Linguistic Variations?

Open-vocabulary audio language models (ALMs), like Contrastive Language Audio Pretraining (CLAP), represent a promising new paradigm for audio-text retrieval using natural language queries. In this paper, for the first time, we perform controlled experiments on various benchmarks to show that existing ALMs struggle to generalize to linguistic variations in textual queries. To address this issue, we propose RobustCLAP, a novel and compute-efficient technique to learn audio-language representations agnostic to linguistic variations. Specifically, we reformulate the contrastive loss used in CLAP architectures by introducing a multi-view contrastive learning objective, where paraphrases are treated as different views of the same audio scene and use this for training. Our proposed approach improves the text-to-audio retrieval performance of CLAP by 0.8%-13% across benchmarks and enhances robustness to linguistic variation.

==> additional_results_best.tex <==
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Retrieval Type $\longrightarrow$}}           & \multicolumn{4}{c}{\textbf{Text-to-Audio Retrieval}}                 & \multicolumn{4}{c}{\textbf{Audio-to-Text Retrieval}}                 \\ \midrule
\multirow{2}{*}{\textbf{Benchmark}}   & \multirow{2}{*}{\textbf{Model}}  & \multicolumn{2}{c}{R@1 $\uparrow$} & \multicolumn{2}{c}{R@10 $\uparrow$} & \multicolumn{2}{c}{R@1 $\uparrow$} & \multicolumn{2}{c}{R@10 $\uparrow$}  \\ \cmidrule(l){3-10} 
                             &                        & TEST & TEST-P & TEST & TEST-P & TEST & TEST-P & TEST & TEST-P   \\ \midrule
\multirow{2}{*}{AudioCaps}   & CLAP                   & \textbf{07.02}           & 04.62            & 48.71         & 35.72           & \textbf{08.78}           & 05.35            & \textbf{49.15}         & 29.72           \\
                             & RobustCLAP             & 06.50          & \textbf{05.89}            & \textbf{49.49}         & \textbf{46.94}           & 07.48           & \textbf{07.71}            & 46.56         & \textbf{43.80}            \\ \midrule
\multirow{2}{*}{Clotho}      & CLAP                   & 38.08          & 30.90            & 81.24         & 75.88           & 37.03          & 30.72           & 81.91         & 74.83           \\
                             & RobustCLAP             & \textbf{38.27}         & \textbf{37.12}           & \textbf{81.53}         & \textbf{80.76}           & \textbf{39.43}         & \textbf{37.32}           & \textbf{82.49}         & \textbf{82.30}           \\ \midrule
\multirow{2}{*}{Audioset SL} & CLAP                   & 12.78          & 11.83           & 48.20          & 42.76           & \textbf{16.52}          & 11.90            & \textbf{52.75}         & 43.71           \\
                             & RobustCLAP             & \textbf{15.77}         & \textbf{14.89}           & \textbf{49.83}         & \textbf{47.52}           & 15.84         & \textbf{14.41}           & 50.37         & \textbf{47.99 }          \\ \midrule
\multirow{2}{*}{SoundDesc}   & CLAP                   & 04.95           & 03.66            & 21.91         & 16.95           & 03.23           & 02.34            & 17.75         & 13.63           \\
                             & RobustCLAP             & \textbf{05.45}          & \textbf{04.12}            & \textbf{23.05}         & \textbf{20.83}          & \textbf{03.78}          & \textbf{02.95}            & \textbf{19.08}         & \textbf{16.92}           \\ \midrule
\multirow{2}{*}{DCASE}       & CLAP                   & 15.05          & 11.84           & 49.25         & 42.63           & 17.25          & 10.93           & \textbf{54.86}         & 43.53           \\
                             & RobustCLAP             & \textbf{16.75}         & \textbf{14.54}           & \textbf{54.26}         & \textbf{49.75}           & \textbf{14.84}         & \textbf{13.14}           & 48.65         & \textbf{45.94}           \\ \bottomrule
\end{tabular}}
\caption{\small T-A and A-T retrieval results for CLAP and RobustCLAP across the original test set (TEST) and the paraphrased test sets (TEST-P). We observe for this new variant of CLAP (630k-fusion-best) again across the benchmark there is a consistent and considerable drop in retrieval performance. When we derive RobustCLAP from this CLAP variant, we again notice the trend where there is improvement in general retrieval recall on \textbf{TEST} and mitigation of the drop in score in TEST-P. The best scores for each benchmark are highlighted in \textbf{bold}. This CLAP variant can be found here: \url{https://huggingface.co/lukewys/laion_clap/blob/main/630k-fusion-best.pt}}
\label{tab:main_result_additional}
\end{table*}



